Shallow or Deep? An Empirical Study on Detecting Vulnerabilities using Deep Learning

Deep learning (DL) techniques are on the rise in the software engineering research community. More and more approaches have been developed on top of DL models, also due to the unprecedented amount of software-related data that can be used to train these models. One of the recent applications of DL in the software engineering domain concerns the automatic detection of software vulnerabilities. While several DL models have been developed to approach this problem, there is still limited empirical evidence concerning their actual effectiveness especially when compared with shallow machine learning techniques. In this paper, we partially fill this gap by presenting a large-scale empirical study using three vulnerability datasets and five different source code representations (i.e., the format in which the code is provided to the classifiers to assess whether it is vulnerable or not) to compare the effectiveness of two widely used DL-based models and of one shallow machine learning model in (i) classifying code functions as vulnerable or non-vulnerable (i.e., binary classification), and (ii) classifying code functions based on the specific type of vulnerability they contain (or "clean", if no vulnerability is there). As a baseline we include in our study the AutoML utility provided by the Google Cloud Platform. Our results show that the experimented models are still far from ensuring reliable vulnerability detection, and that a shallow learning classifier represents a competitive baseline for the newest DL-based models.

==> secs/highlights.tex <==
\textcolor{blue}{
Based on the experience earned by conducting the empirical study and complemented with the results, we have the following highlights for researchers and practitioners. 
}
%Concerning \emph{Data Collection and labeling}, in data-driven approaches the main asset and a key factor is the data, specially the training data which helps our systems to learn and make accurate decisions and predictions. This learning strategy is based on identifying patterns and associations in historical training data, therefore, with high-quality data the overall performance of our data-driven approaches may be enhanced. It is challenging to find useful sets of data for such purposes, however, nowadays mining software repositories is a feasible task given the increasing number of open source projects publicly available, thus the community has created and released a wide range of annotated and curated data sets of different nature (\ie real-world and synthetic data), being convenient for devising DL-techniques in the context of Software Engineering field. Nevertheless, some challenges remain, \ie in the context of this study, the amount of vulnerable instances can be less than non-vulnerable data points, creating an issue about the imbalanced nature of the data set thus leading to marred results, therefore is important to consider such characteristics while deciding which metrics are going to be used within the evaluation stage, since it could lead to misleading conclusions.

%\textcolor{blue}{
%Referring to \emph{Code Representation}, even though some of the best results we obtained are related to abstracts representations having more syntactic and semantic meaning of tokens structuring each function, we cannot claim based on our empirical evidence and results, that as long as there is more contextual information the overall performance of the models will increase, on the contrary in the literature one can appreciate that over-fitting models are related to the few amount of data training instances and their particular characteristics (\eg syntactic and semantics attributes).
%}


\textcolor{blue}{
Regarding the \emph{Classifiers}, it is important to highlight that we followed two types of process concerning the training and tuning models, namely manual and automatic approaches. Concerning the former, we specifically established the searching space for hyper-parameters tuning and we also transform our original abstract representations to a sequence or BOW representation. On the other hand, referring to the latter and in respect to AutoML, we upload the original abstract representations to the platform and it modifies the input if needed, deciding also the hyper-parameters to be tuned. AutoML reduces human interaction in the process of finding a good model, however, if we wanted to analyze the model's architecture or the concrete input, it would be not possible given its black-box approach, moreover, for AutoML-NLP in GCP it is not possible to download a model and deploy it locally, thus incurring in extra costs for deploying a model and making classifications of documents. During the process of training in GCP we found that this platform has some tutorials about how to use it, but it lacks good documentation of how it works, leading us to search documentation of similar services to AutoML for NLP, like AutoML-Tables, which has a more complete documentation. Another interesting point regarding classifiers, is that if we evaluate precision, as the decision metric,  in some case we had a tie between RF and DL models (\eg  binary, R0, J-DS), in which due to Occam's Razor principle\cite{NIPS2000_0950ca92} we should choose RF since it is the least complex model that learnt the target function.
}


\textcolor{blue}{
	In respect of \emph{Analysis method},  it is important to establish a set of metrics allowing to make well-informed decisions, this is the case of R-DS multi-class classifiers, taking only into account Accuracy is not possible to see how precise is the model for all the classes. Furthermore,  in multi-class classification we found that not always the type of average is presented in the state-of-art \cite{Li2018}, and that could lead to a misunderstanding of the models performance, since each type of average can be interpreted differently (\ie macro-average gives the same importance to each class being insensitive to class imbalance, while micro average maximize hits).  
}



==> secs/sb_cleaning_classifiers_abnalysis.tex <==
% !TEX root = empirical_study.tex
\subsection{Data Cleaning}
Before using the built datasets to train and evaluate the experimented models, we performed a transformation and cleaning process on each of them to (i) make the data treatable with DL models, and (ii) avoid possible pitfalls that are common in studies of machine learning on code (\eg duplicated functions due to forked projects \cite{Allamanis:MSR13, Allamanis:18}). 

First, for each dataset we created different versions using the five code representations shown in \figref{representations}. This gave us five different datasets of function representations for each dataset.

{\color{blue}
Second, we addressed duplicates and conflicting representation (\ie for single-label classification two samples with same code representation and different labels). We considered  duplicated sample  if more than one sample had the same code representation+extra information with the same label. This extra information, helps us to understand the uniqueness of the representation, \eg  for each J-DS was the flow variant, GH-DS was SHA number and R-DS did not has extra information. In case of duplicates, only the first occurrence was conserved. As for the conflicting representations, all instances were removed. Note that duplicates and conflicting instances can be different in the same dataset when using different representations. For example, two functions can be different using the more expressive R4 representation and equal when using the basic R0 representation. In this case, the duplicate will be removed from the dataset only when using the R0 representation. \tabref{tab:duplicatedData} summarizes the final number of functions in each dataset after this process. It is important to mention that after this process GH-DS is no longer balanced.  }


%Duplicate representations, in the GH-DS, were identified after analyzing that for each year we found commits across different repositories having same SHAs, and sharing the same changes applied to the same files (leading to the same representation). Equal representations with same SHA, that had more than one label, were considered as conflicting representations. In J-DS samples were only considered as duplicate if the representation is the same and they are part of the same flow variation. No conflicting representation were found for J-DS. Concerning R-DS, the functions in this dataset also contain cloned functions that become identical when using some of the code representations in \figref{representations}, also conflicting labeled functions were found. \GABRIELE{Removed, these are very technical details}



\begin{table}[t]
	\caption{Number of functions in each dataset for each representation after handling duplicates and conflicting representations. \ANA{myself Verify these numbers}}
	\label{tab:duplicatedData}
	\centering
	\begin{tabular}{lrrr}
		\toprule
		 & GH-DS & J-DS & R-DS\\
		\midrule
		R0  & 164,919 & 56,073 & 1,117,137\\
		R1  & 166,187 & 56,075 & 1,117,765\\
		R2  & 167,280 & 56,083 & 1,117,925\\
		R3  & 172,421 & 56,075 & 1,118,349\\
		R4  & 173,498 & 56,083 & 1,118,488\\
\bottomrule
	\end{tabular}
	\vspace{-1\baselineskip}
\end{table}

Third, for each dataset, we computed the distribution of number of tokens for all functions representations it contains. Then, for each dataset representation, we excluded functions that are shorter than the first quartile (\eg for R1 J-DS 59 tokens) or longer than the third quartile (\eg for R1 J-DS 115 tokens). This has been done to exclude very short and very long functions from our dataset since the former provide very little information to characterize the presence of a vulnerability and the second are computationally expensive to process with DL models. Another possibility, often applied in DL-based studies, is sequence truncation during the training phase. This  consists in trimming long sentences to a fixed numbers. This approach has the drawback of providing incomplete inputs to the model, something suboptimal when working with source code. Thus, this preprocessing step aims at mitigating this issue by removing upfront very long functions. After this step, the data cleaning process for binary classification ends, and the final number of functions for this type of classification can be seen in \tabref{tab:cleanedDataB}. 

\begin{table}[t]
	\caption{Number of functions in each dataset for each representation after data cleaning for binary classification.}
	\label{tab:cleanedDataB}
	\centering
	\begin{tabular}{lrrr}
		\toprule
		 & GH-DS & J-DS & R-DS\\
		\midrule
		R0  & 70,618 & 28,572 & 563,646\\
		R1  & 71,757 & 28,572 & 563,752\\
		R2  & 72,214 & 28,572 & 563,817\\
		R3  & 79,216 & 28,572 & 563,923\\
		R4  & 79,545 & 28,572 & 563,970\\
\bottomrule
	\end{tabular}
	%\vspace{-1\baselineskip}
\end{table}

Finally, to have enough data points to train the multi-class models in charge of identifying the specific type of vulnerability affecting a given function, we kept in each dataset only the five most represented vulnerabilities and non-vulnerable (see \tabref{tab:topFive}). Note that this was only needed for GH-DS and J-DS, since R-DS does already focus on four possible categories of vulnerabilities. In R-DS one of the possible categories (CWE-119), after the cleaning process, had only five samples and we decided to merge it with another category (CWE-120), since representing similar vulnerabilities. \tabref{tab:cleanedDataM} summarizes the final number of functions for multi-class classification. 


\begin{table}[t]
	\caption{Top five vulnerabilities in each dataset. *Russell has only four vulnerabilities, and two of them were merged}
	\label{tab:topFive}
	\centering
	\begin{tabular}{p{0.06 \textwidth}p{0.37  \textwidth}}
		\toprule
		 Dataset& Top Vulnerabilities \\
		\midrule
		GH-DS  & Deadlock, Race Condition, Null Pointer Dereference, Buffer Overflow, Dead Code\\
		J-DS   & CWE-401, CWE-762, CWE-590, CWE-122, CWE-121 \\
		R-DS*   & CWE-other, CWE-120, CWE-476\\
\bottomrule
	\end{tabular}
	%\vspace{-1\baselineskip}
\end{table}


\begin{table}[t]
	\caption{Number of functions in each dataset for each representation after data cleaning for multi-class classification.}
	\label{tab:cleanedDataM}
	\centering
	\begin{tabular}{lrrr}
		\toprule
		 & GH-DS & J-DS & R-DS\\
		\midrule
		R0  & 57,475 & 11,445 & 563,646\\
		R1  & 57,947 & 11,445 & 563,752\\
		R2  & 58,390 & 11,445 & 563,817\\
		R3  & 60,305 & 11,445 & 563,923\\
		R4  & 60,768 & 11,445 & 563,970\\
\bottomrule
	\end{tabular}
	%\vspace{-1\baselineskip}
\end{table}

At the end of this process we obtained 30 different datasets. The first 15 datasets correspond to the binary classification, whereby the labels can only take two possible values (vulnerable or non-vulnerable). The other 15 datasets correspond to the multiclass classification and their labels represent a specific type of vulnerability or a non-vulnerable instance. {\color{blue} In addition, remember that within the datasets we had a special kind of duplicates related to different functions having the same abstract representation, they were not removed since the extra information added to analyze their uniqueness kept them as unique however, particularly for GCP training process, we must delete these remaining duplicated instances in order to upload the dataset GCP since this platform considers them as errors.}

\subsection{Classifiers}

{\color{blue}Given the variables involved in our study (three-fold process, three models, five representations, three datasets, and two types of classification---binary and multiclass), we had to build 90 models for the first stage and ($3*5*3*2$) and 75 models for the remaining two stages. Thus being 165 models in total.}

{\color{blue}As previously mentioned, in our first round we trainned our base line model (RF), that uses shallow learning, and the two aformentioned deep learning models (CNN a RNN, specifically an LSTM). } Concerning the RF, for binary and multi-class classification the model is the same, with the only difference being the labels in the training/test set. We used a balanced class weighting to contrast imbalanced classes. For this model the input data is a Bag of words (BOW) of the specific representation and the output is a label classifying the instance. We used Scikit learn \cite{sklearn_api} implementation and the hyper-parameters that we tuned are reported in \tabref{tab:HyperParameters}.

\begin{table}[t]
	\caption{Hyper-parameters that were tuned for each type of model.}
	\label{tab:HyperParameters}
	\centering
	\begin{tabular}{p{0.06 \textwidth}p{0.37  \textwidth}}
		\toprule
		 Model & Hyper-parameters tuned\\
		\midrule
		RF  & Number of estimators, Number of features to consider at every split, Maximum  number of levels in tree, Function used to evaluate the quality of a split\\
		CNN  & Dimension of the dense embedding, Number of output filters, Length of the convolution window, Stride Length of the convolution, Initializer for the kernel weights matrix, Activation function for convolution layer, Regularizing factor applied to the kernel weights matrix, Drop out rate, Number of dense layers, Activation function for each dense layer, Numbers of neurons for each dense layer, Optimizer, Optimizer's learning rate, Batch size\\
		RNN  & Dimension of the dense embedding, Dimensionality  of the output space, Activation function    for recurrent layer, Initializer for the recurrent kernel weights matrix, Initializer for the kernel weights matrix, Regularizing factor for the kernel weights matrix, Regularizing factor for the recurrent kernel weights matrix, Drop out rate, Optimizer, Optimizer's learning rate, Batch size  \\
\bottomrule
	\end{tabular}
	%\vspace{-1\baselineskip}
\end{table}


For the RNN \cite{RUSSELL, Li2018, Li20182, LIN2019} and CNN  \cite{RUSSELL, FWU2017, Li20182, HARER2018} models, the input layer takes as input a token sequence extracted from the specific code representation and converts it into a fixed $k$-dimensional  embedding representation. The $k$ value is one of the hyper-parameters to tune. The output layer is a one-hot encoded vector that corresponds to a particular label. For the binary case the output layer has sigmoid activation function and one neuron, for multi-class case it uses a softmax activation function and the number of neurons is equivalent to the number of prediction classes (\eg for R-DS the output layer has 4 neurons, but for J-DS it uses six neurons). The hidden layers between the input and output layers differ between these two models.

For the CNN, after the embedding layer, we a have one dimensional convolutional layer, since we are working with one dimensional data (text), as opposed to other contexts in which more dimensions are needed (\eg to manipulate images). The hyper-parameters that we tune for this layer are:  the number of filters, the kernel size and  the activation function. After this layer, the CNN model includes a global max pooling layer, a drop out layer (to reduce the chance of overfitting) with a rate that can be tuned, and one or two dense layers depending on the hyper-parameter optimization process.

The RNN has a LSTM layer after the embedding layer. The hyper-parameters we tune for this layer are:  the number of units and the initialization of the kernels and the activation function. After this layer, also the RNN uses a drop out layer to prevent over fitting. 

For both CNN and RNN, the learning rate and the batch size were also hyper-parameters to tune. We also experimented with both the Adam and Nadam optimizers. For both models, CNN and RNN, we used Keras \cite{chollet2015keras}. 

{\color{blue}
For the second round we continue training  RNN and CNN models for which we also tuned the aformentioned parameters. For the last round with GCP, we could not choose or known  which types of models were trained or which was the search space for each model. For this round we only upload the plai text representation with labels and an identifier indicating if the data belong to train, validation or test data. }

\input{secs/analysis}

==> tables/tabBinary.tex <==
% !TEX root = results.tex

\begin{table*}[]
	\caption{Binary metrics,Precision (P), Recall (R) and F1 for each dataset-representation and the two approaches of tunning the DL model. using vulnerable as the positive class \ANA[missing]{AutoML?}}
	\label{tab:resultsBinary}
	\scalebox{0.8}{
		{\color{blue}
			\begin{tabular}{lc|ccc|ccc|ccc|ccc|ccc}
				&
				\textbf{} &
				\multicolumn{3}{|c|}{\textbf{CNN-1}} &
				\multicolumn{3}{|c|}{\textbf{RNN-1}} &
				\multicolumn{3}{|c|}{\textbf{RF}} &
				\multicolumn{3}{|c|}{\textbf{CNN-2}} &
				\multicolumn{3}{c}{\textbf{RNN-2}} \\
				&
				\textbf{Rep} &
				\textbf{P} &
				\textbf{R} &
				\textbf{F1} &
				\textbf{P} &
				\textbf{R} &
				\textbf{F1} &
				\textbf{P} &
				\textbf{R} &
				\textbf{F1} &
				\textbf{P} &
				\textbf{R} &
				\textbf{F1} &
				\textbf{P} &
				\textbf{R} &
				\textbf{F1} \\
				\midrule
				\multicolumn{1}{c}{\multirow{5}{*}{\textbf{J-DS}}} &
				1 &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				99.58\% &
				99.79\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% \\
				\multicolumn{1}{c}{} &
				2 &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				99.88\% &
				99.94\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% \\
				\multicolumn{1}{c}{} &
				3 &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				99.76\% &
				99.88\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% \\
				\multicolumn{1}{c}{} &
				4 &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				99.70\% &
				99.85\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% \\
				\multicolumn{1}{c}{} &
				5 &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				99.76\% &
				99.88\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% &
				100\% \\
				\multirow{5}{*}{\textbf{GH-DS}} &
				1 &
				55.83\% &
				78.32\% &
				65.19\% &
				51.08\% &
				92.47\% &
				65.81\% &
				63.87\% &
				63.80\% &
				63.84\% &
				100.00\% &
				64.15\% &
				63.43\% &
				52.21\% &
				54.66\% &
				53.41\% \\
				&
				2 &
				60.12\% &
				53.12\% &
				56.40\% &
				68.95\% &
				2.66\% &
				5.12\% &
				61.30\% &
				62.18\% &
				61.73\% &
				65.71\% &
				65.58\% &
				65.65\% &
				54.29\% &
				16.66\% &
				25.49\% \\
				&
				3 &
				57.51\% &
				63.69\% &
				60.45\% &
				52.86\% &
				45.75\% &
				49.05\% &
				60.45\% &
				60.75\% &
				60.60\% &
				61.20\% &
				62.67\% &
				61.92\% &
				50.49\% &
				92.91\% &
				65.43\% \\
				&
				4 &
				59.16\% &
				58.97\% &
				59.06\% &
				61.85\% &
				80.08\% &
				69.79\% &
				63.04\% &
				78.79\% &
				70.04\% &
				61.71\% &
				62.55\% &
				62.13\% &
				62.52\% &
				97.28\% &
				76.12\% \\
				&
				5 &
				58.65\% &
				62.37\% &
				60.46\% &
				50.74\% &
				74.62\% &
				60.40\% &
				59.59\% &
				89.42\% &
				71.52\% &
				63.18\% &
				64.80\% &
				63.98\% &
				50.87\% &
				35.52\% &
				41.83\% \\
				\multirow{5}{*}{\textbf{R-DS}} &
				1 &
				32.65\% &
				4.78\% &
				8.34\% &
				38.85\% &
				12.95\% &
				19.42\% &
				11.27\% &
				50.31\% &
				18.42\% &
				74.14\% &
				0.99\% &
				1.95\% &
				62.70\% &
				1.82\% &
				3.53\% \\
				&
				2 &
				33.23\% &
				7.15\% &
				11.77\% &
				37.54\% &
				19.89\% &
				26.00\% &
				11.10\% &
				52.23\% &
				18.31\% &
				72.58\% &
				1.03\% &
				2.04\% &
				53.21\% &
				2.67\% &
				5.08\% \\
				&
				3 &
				30.92\% &
				5.31\% &
				9.06\% &
				33.78\% &
				18.18\% &
				23.64\% &
				11.29\% &
				50.86\% &
				18.48\% &
				61.19\% &
				0.94\% &
				1.86\% &
				50.55\% &
				3.15\% &
				5.93\% \\
				&
				4 &
				23.61\% &
				10.16\% &
				14.21\% &
				31.10\% &
				20.23\% &
				24.51\% &
				52.12\% &
				5.38\% &
				9.75\% &
				61.71\% &
				1.08\% &
				2.12\% &
				50.43\% &
				2.69\% &
				5.10\% \\
				&
				5 &
				31.41\% &
				5.88\% &
				9.91\% &
				32.26\% &
				15.47\% &
				20.91\% &
				12.06\% &
				45.30\% &
				19.05\% &
				62.07\% &
				1.24\% &
				2.43\% &
				48.32\% &
				2.64\% &
				5.01\%
		\end{tabular}}
	}
\end{table*}



==> tables/tabMulti.tex <==
% !TEX root = results.tex

\begin{table*}[h]
		\caption{ Macro Precision (P),macro Recall (R) , macro F1  and Accyracy for each dataset-representation and the two approaches of tunning the DL model \ANA[missing]{AutoML?}}
	\label{tab:resultsMulti}
	
	\scalebox{0.6}{
	{\color{blue}
	\begin{tabular}{lccccc|cccc|cccc|cccc|cccc}
		&
		\textbf{} &
		\multicolumn{4}{|c|}{\textbf{CNN-1}} &
		\multicolumn{4}{c|}{\textbf{RNN-1}} &
		\multicolumn{4}{c|}{\textbf{RF}} &
		\multicolumn{4}{c|}{\textbf{CNN-2}} &
		\multicolumn{4}{|c}{\textbf{RNN-2}} \\
		&
		\multicolumn{1}{l|}{} &
		&
		\multicolumn{3}{|c|}{\textbf{Macro}} &
		&
		\multicolumn{3}{|c|}{\textbf{Macro}} &
		&
		\multicolumn{3}{|c|}{\textbf{Macro}} &
		&
		\multicolumn{3}{|c|}{\textbf{Macro}} &
		&
		\multicolumn{3}{|c}{\textbf{Macro}} \\
		&
		\textbf{Rep} &
		\multicolumn{1}{|c|}{\textbf{ACC}} &
		\multicolumn{1}{c}{\textbf{P}} &
		\multicolumn{1}{c}{\textbf{R}} &
		\multicolumn{1}{c|}{\textbf{F1}} &
		\multicolumn{1}{l|}{\textbf{ACC}} &
		\multicolumn{1}{c}{\textbf{P}} &
		\multicolumn{1}{c}{\textbf{R}} &
		\multicolumn{1}{c|}{\textbf{F1}} &
		\multicolumn{1}{l|}{\textbf{ACC}} &
		\multicolumn{1}{c}{\textbf{P}} &
		\multicolumn{1}{c}{\textbf{R}} &
		\multicolumn{1}{c|}{\textbf{F1}} &
		\multicolumn{1}{l|}{\textbf{ACC}} &
		\multicolumn{1}{c}{\textbf{P}} &
		\multicolumn{1}{c}{\textbf{R}} &
		\multicolumn{1}{c|}{\textbf{F1}} &
		\multicolumn{1}{l|}{\textbf{ACC}} &
		\multicolumn{1}{c}{\textbf{P}} &
		\multicolumn{1}{c}{\textbf{R}} &
		\multicolumn{1}{c}{\textbf{F1}} \\ \hline
		\multicolumn{1}{c}{} &
		\multicolumn{1}{c|}{1} &
		 96.16 &
		 92.38 &
		 90.07 &
		 91.08 &
		 99.87 &
		 99.70 &
		 99.60 &
		 99.65 &
		 99.69 &
		 99.72 &
		 99.14 &
		 99.42 &
		 99.52 &
		 99.00 &
		 98.69 &
		 98.84 &
		 99.96 &
		 99.79 &
		 99.93 &
		 99.86 \\
		\multicolumn{1}{c}{} &
		\multicolumn{1}{c|}{2} &
		 98.25 &
		 94.50 &
		 96.44 &
		 95.25 &
		 98.30 &
		 95.31 &
		 95.41 &
		 95.35 &
		 99.69 &
		 99.71 &
		 99.19 &
		 99.45 &
		 99.87 &
		 99.69 &
		 99.51 &
		 99.60 &
		 99.83 &
		 99.59 &
		 99.44 &
		 99.51 \\
		\multicolumn{1}{c}{} &
		\multicolumn{1}{c|}{3} &
		 98.21 &
		 95.49 &
		 94.62 &
		 95.03 &
		 99.83 &
		 99.59 &
		 99.59 &
		 99.59 &
		 99.96 &
		 99.79 &
		 99.93 &
		 99.86 &
		 99.87 &
		 99.69 &
		 99.65 &
		 99.67 &
		 99.83 &
		 99.63 &
		 99.68 &
		 99.66 \\
		\multicolumn{1}{c}{} &
		\multicolumn{1}{c|}{4} &
		 98.95 &
		 97.16 &
		 97.20 &
		 97.18 &
		 99.30 &
		 98.44 &
		 98.09 &
		 98.26 &
		 99.83 &
		 99.75 &
		 99.39 &
		 99.57 &
		\multicolumn{1}{c}{ 100} &
		\multicolumn{1}{c}{ 100} &
		\multicolumn{1}{c}{ 100} &
		\multicolumn{1}{c|}{ 100} &
		 99.83 &
		 99.74 &
		 99.49 &
		 99.61 \\
		\multicolumn{1}{c}{\multirow{-5}{*}{\textbf{J-DS}}} &
		\multicolumn{1}{c|}{5} &
		 99.13 &
		 97.74 &
		 97.87 &
		 97.79 &
		 97.77 &
		 94.63 &
		 95.09 &
		 94.69 &
		 99.83 &
		 99.70 &
		 99.54 &
		 99.62 &
		 99.96 &
		 99.79 &
		 99.93 &
		 99.86 &
		 99.87 &
		 99.57 &
		 99.80 &
		 99.68 \\
		&
		\multicolumn{1}{c|}{1} &
		 50.35 &
		 53.51 &
		 19.27 &
		 16.44 &
		 49.54 &
		 8.26 &
		 16.67 &
		 11.04 &
		 64.71 &
		 65.07 &
		 57.63 &
		 60.77 &
		 54.08 &
		 65.38 &
		 25.85 &
		 27.34 &
		 57.58 &
		 54.20 &
		 41.28 &
		 44.31 \\
		&
		\multicolumn{1}{c|}{2} &
		 50.91 &
		 57.99 &
		 20.55 &
		 18.79 &
		 49.58 &
		 8.26 &
		 16.67 &
		 11.05 &
		 62.36 &
		 61.80 &
		 54.97 &
		 57.82 &
		 53.54 &
		 57.04 &
		 28.03 &
		 30.92 &
		 54.67 &
		 45.38 &
		 34.41 &
		 37.21 \\
		&
		\multicolumn{1}{c|}{3} &
		 55.11 &
		 55.09 &
		 31.43 &
		 34.92 &
		 49.59 &
		 8.27 &
		 16.67 &
		 11.05 &
		 63.14 &
		 63.08 &
		 55.29 &
		 58.49 &
		 56.78 &
		 55.01 &
		 39.92 &
		 44.35 &
		 57.24 &
		 52.13 &
		 47.74 &
		 49.44 \\
		&
		\multicolumn{1}{c|}{4} &
		 53.10 &
		 64.28 &
		 23.28 &
		 23.25 &
		 49.81 &
		 8.30 &
		 16.67 &
		 11.08 &
		 60.79 &
		 59.93 &
		 51.21 &
		 54.70 &
		 56.37 &
		 54.41 &
		 34.50 &
		 38.14 &
		 54.54 &
		 48.23 &
		 38.35 &
		 40.64 \\
		\multirow{-5}{*}{\textbf{GH-DS}} &
		\multicolumn{1}{c|}{5} &
	 54.00&
	 46.73 &
	 37.04 &
	 39.26 &
	 49.82 &
	 8.30 &
	 16.67 &
	 11.08 &
	 61.23 &
	 60.43 &
	 51.64 &
	 55.17 &
	 54.13 &
	 48.06 &
	 39.16 &
	 41.90 &
	 57.71 &
	 54.15 &
	 33.07 &
	 35.89 \\
		&
		\multicolumn{1}{c|}{1} &
	 48.08\% &
	 39.52\% &
	 14.41\% &
	 20.02\% &
	 48.07\% &
	 6.02\% &
	 6.13\% &
	 6.07\% &
	 24.19\% &
	 24.97\% &
	 8.37\% &
	 9.68\% &
	 96.15\% &
	 37.44\% &
	 27.00\% &
	 28.00\% &
	 96.16\% &
	 38.75\% &
	 26.76\% &
	 27.68\% \\
		&
		\multicolumn{1}{c|}{2} &
	 48.07\% &
	 45.00\% &
	 14.90\% &
	 20.68\% &
	 48.07\% &
	 24.04\% &
	 12.25\% &
	 16.23\% &
	 48.11\% &
	 72.96\% &
	 16.82\% &
	 24.14\% &
	 96.15\% &
	 37.80\% &
	 26.94\% &
	 27.92\% &
	 96.17\% &
	 56.49\% &
	 28.10\% &
	 29.70\% \\
		&
		\multicolumn{1}{c|}{3} &
	 48.07\% &
	 70.47\% &
	 13.25\% &
	 18.14\% &
	 48.07\% &
	 24.04\% &
	 12.25\% &
	 16.23\% &
	 48.13\% &
	 78.55\% &
	 16.88\% &
	 24.41\% &
	 96.17\% &
	 53.53\% &
	 27.04\% &
	 28.19\% &
	 96.19\% &
	 66.97\% &
	 27.40\% &
	 28.76\% \\
		&
		\multicolumn{1}{c|}{4} &
		 48.08\% &
	    39.10\% &
		13.81\% &
	   19.07\% &
		 48.07\% &
		 24.04\% &
		 12.25\% &
		 16.23\% &
	     48.11\% &
		 77.44\% &
		 15.51\% &
		 22.19\% &
		 96.19\% &
		 65.58\% &
		 28.83\% &
		 31.27\% &
		 96.15\% &
		 48.10\% &
		 27.96\% &
		 29.76\% \\
		\multirow{-5}{*}{\textbf{R-DS}} &
		\multicolumn{1}{c|}{5} &
		 48.08\% &
		 39.70\% &
		 14.23\% &
		 19.74\% &
		 48.07\% &
		 6.02\% &
		 6.13\% &
		 6.07\% &
		 48.11\% &
		 73.49\% &
		 16.16\% &
		 23.14\% &
		 96.17\% &
		 39.31\% &
		 27.44\% &
		 28.73\% &
		 96.16\% &
		 48.66\% &
		 28.23\%&
		29.90\%
	
	\end{tabular}}

}
\end{table*}
